SPHERE-JEPA: Spherical Prediction with Homogeneous Embeddings

A fundamental open question in self-supervised learning (SSL) is the explicit characterization of the optimal geometry of the learned representations. Recently, LeJEPA identified isotropic Gaussian embeddings as optimal for minimizing downstream prediction risk in Euclidean spaces. However, the corresponding problem for distributions supported on lower-dimensional manifolds, such as the hypersphere, remains unexplored. In this work, we demonstrate that extending this minimax analysis to smooth distributions on Riemannian manifolds fundamentally changes the optimal solution. We show that, under a worst-case formulation, both k-nearest neighbors and kernel ridge regression induce hyperspherical uniformity. More precisely, we show that uniform distributions on manifolds are optimal for k-nearest neighbors, and that the uniform distribution on the sphere is optimal for kernel ridge regression with both the exponential dot-product kernel and the linear kernel. This theoretical insight reveals a fundamental limitation of Gaussian embeddings: their non-uniform density induces anisotropic k-NN neighborhoods, severely biasing the estimator. To correct this, we introduce SPHERE-JEPA, a theoretically grounded SSL framework. We adapt LeJEPA's Cram{\'e}r-Wold projection mechanism to enforce hyperspherical uniformity rather than a Gaussian prior. Empirically, SPHERE-JEPA yields significant improvements, boosting texture retrieval mAP by over 6%, while consistently matching or outperforming LeJEPA on standard benchmarks-including a +1.8% linear probing gain on ImageNet-1K (ViT-B/14).

==> Makefile <==
PDF  != ls *.tex | sed 's/\.tex/.pdf/'
pdf   : $(PDF)
%.pdf : %.tex ; cat $< | bash pdflatexfilter > $@
clean :       ; $(RM) $(PDF)


==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
%The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page limit. 

%Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
%\begin{itemize}
%    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%    \item Please provide a short (1--2 sentence) justification right after your answer (even for \answerNA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
%\end{itemize}

%{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will also be asked to include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

%The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While \answerYes{} is generally preferable to \answerNo{}, it is perfectly acceptable to answer \answerNo{} provided a proper justification is given (e.g., error bars are not reported because it would be too computationally expensive'' or ``we were unable to find the license for the dataset we used''). In general, answering \answerNo{} or \answerNA{} is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

%IMPORTANT, please:
%\begin{itemize}
%    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
%    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
%\end{itemize} 
 

%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item {\bf Claims}
\item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
\item[] Answer: \answerYes{}
\item[] Justification: The abstract and introduction explicitly state our theoretical contributions regarding hyperspherical optimality (detailed in Section 4) and accurately summarize the supporting empirical results on standard and retrieval benchmarks (detailed in Section 6).
\item[] Guidelines:
\begin{itemize}
    \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
    \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
    \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
    \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
\end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: Empirical limitations—specifically our reliance on a single training run without hyperparameter tuning, and the need to scale to larger batch sizes and architectures—are explicitly acknowledged in the Conclusion (Section 7).
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{}
    \item[] Justification: All geometric and topological assumptions are explicitly stated in the main text within the statements of Lemma 1 and Theorem 1 (Section 4). The complete and formal proofs for these results are provided in the supplemental material (Appendix).
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

\item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification: The experimental setup, including architectures, augmentations, and hyperparameters, is detailed in Section 6 and the Appendix. Furthermore, we will release a GitHub repository containing the core implementation of SUSReg and the specialized texture retrieval dataset upon publication.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}
    \item[] Justification: We provide an anonymized ZIP file in the supplementary material containing the core PyTorch implementation of the SUSReg loss and the custom texture retrieval dataset. The full training pipeline will be open-sourced upon publication.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: All critical experimental details, including datasets, model architectures, optimizer choices, data augmentation strategies, and specific hyperparameter values (e.g., learning rates, batch sizes, EMA momentum) are thoroughly described in Section 6. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{}
    \item[] Justification: Due to the high computational cost of pretraining large vision backbones (e.g., ViT-B/14) on large-scale datasets (ImageNet-1K), our main results report metrics from a single training run. We explicitly acknowledge the absence of multi-seed robustness evaluation as a limitation in Section 7.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: We provide complete details regarding the hardware specifications (NVIDIA A100 80GB and RTX-6000 GPUs) and training execution times (e.g., 2.5 days for ViT-B/14 on ImageNet-1K) in the Computational Resources section of the Appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    \item[] Justification: The research focuses on foundational methodology and theoretical geometry for self-supervised learning. It relies solely on standard, publicly available datasets and does not involve human subjects, sensitive information, or immediately harmful applications.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{}
    \item[] Justification: Our work is strictly foundational and theoretical, focusing on the geometry of optimal representations in self-supervised learning. It does not propose a specific application or deployment, and therefore does not have direct societal impacts to discuss.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
    \item[] Justification: Our research focuses on foundational vision encoders for representation learning, rather than generative models or large language models. The provided models and the custom texture dataset do not pose a high risk for misuse, such as the generation of unsafe content or deepfakes.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: All existing datasets (ImageNet, Galaxy10) and software libraries (PyTorch) used in our work are properly cited in Section 6. A brief discussion of their respective licenses is provided in the Appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{}
    \item[] Justification: We introduce a novel custom texture retrieval dataset and the SPHERE-JEPA/SUSReg codebase. Detailed documentation regarding the dataset structure, evaluation protocols, and code usage is provided in the Appendix and alongside the assets in the anonymized supplementary ZIP file.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}
    \item[] Justification: Our research does not involve crowdsourcing or human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: Our research is purely computational and theoretical; it does not involve human subjects, and therefore IRB approval is not applicable.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    \item[] Answer: \answerNA{}
    \item[] Justification: As LLMs were solely used for writing and editing purposes and are not a component of the core methodology, a formal declaration in the paper is not required according to the guidelines.    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> other.tex <==


\label{appendix:canonical_geometry}
\isb*




\begin{restatable}{prop}{linear}
    
\end{restatable}
\begin{proof}
The linear probe extracts $Y = Z\beta$, where $Z$ is a random variable in $\mathbb{R}^d$ with mean $\mu_Z = 0$ and covariance $C_Z = \mathbb{E}[Z^2]$. Then, for each $\beta\in\mathbb{R}^d$, $Y$ is a zero-mean random variable in $\mathbb{R}$ with covariance $\beta^TC_Z \beta.$ Suppose that we have a prior $p(\beta) = \mathcal{N}(0,\tau^2 I)$.

Given a  posterior estimate of $\beta$,

Since $p(Y=y|Z,\beta) = p(Z\beta = y | Z,\beta) = p$

\end{proof}




\section{Comparing the Covariance Matrices of Neighborhoods of a Point}
While the covariance matrices of both $\mathcal{N}(0,I_d)$ and the uniform distribution on $S^{d-1}$ are both \emph{globally} isotropic, they are locally anisotropic: a covariance matrix computed on data in a neighborhood around some point $p\in\mathbb{R}^d$ (for the Gaussian) and on a spherical cap around $p\in S^{d-1}$ (for the uniform distribution on the sphere) will not be a multiple of the identity.

\paragraph{Standard Gaussian in $\mathbb{R}^d$:}

\paragraph{Uniform distribution on $\mathbb{S}^{d-1}$:} Let $x\sim \text{Unif}(\mathbb{S}^{d-1}$), conditioned on being within a geodesic ball of radius $r$ of some point $p\in \mathbb{S}^{d-1}$, $B_r(p)$. By symmetry, we can take $p$ to be the North Pole $e_1\in\mathbb{R}^d.$ Moreover, by symmetry, the mean vector must be proportional to $p$: $\mathbb{E}[x] = \mu_1 e_1.$ We can parameterize $x=(\cos(\theta), \sin(\theta)u)$ where $u\in\mathbb{S}^{d-2}$ and $\theta$ is the colatitude. In the geodesic ball of radius $r$, $\theta \in [0, r]$, corresponding to coordinate values $x^Te_1 = 1-\cos(\theta)$ and latitudinal line radii $\sin(\theta) $ Thus, since the uniform measure on the sphere $\mathbb{S}^{d-1}$, $d\text{vol}_{d-1}(x)$, decomposes as $\sin^{d-2}\theta d\theta  d\text{vol}_{d-2}(x)$, by azimuthal symmetry, we have
$\mu_1 \propto \int_{B_r(e_1)} d\text{vol}(x) = \int_{0}^r \cos(\theta)\sin^{d-2}(\theta) d\theta =\int_{\cos r}^1 t(1-t^2)^{(d-3)/2}dt = \frac{1}{C}\frac{\sin^{d-1}(r)}{d-1}$ with normalizing constant $C = \int_{\cos(r)}^1 (1-t^2)^{(d-3)/2}dt.$



\paragraph{Conclusion of Theorem~\ref{thm:canonical_geometry}.}
By Step~2, the embedding distribution is uniform on $\mathcal M$.
By Lemma~\ref{lem:Od_invariant_implies_sphere}, $\mathcal M = r\,\mathbb{S}^{d-1}$.
Therefore the unique uniform distribution on $\mathcal M$ is the uniform (Haar) measure
on the hypersphere.
This completes the proof.













\section{Optimality Criteria for Self-Supervised Representations on Riemannian Manifolds} \label{OptimalityRepresentation}


%Mettre le resultsat qui dit que Un minimisateur de knn et de linear probing est la distribution uniforme sur lhyspespere
%Et mettre une remarque qui dit la "verité" Ie detre uniforme sur un manifold riemanien + instropique dans lespace ambient (R^d) 

%\textcolor{red}{For each downstream learning task, the predictor of \citep{balestriero2025lejepaprovablescalableselfsupervised} is a multi-index model on the Gaussian embeddings with filter function $g=\text{id}$; this exact model can be recovered from spherical embeddings using a filter function that normalizes $g(x) = x/||x||_2$\citep{bruna2025survey}.}

%\textcolor{red}{Un minimisateur de knn et linear probing cest la distribution sur lhypersphere}
%\textcolor{red}{Remarque: Enfaite pour etre un minimisateur de knn et linear probingil faut etre une distribution uniforme sur un manifold compact et etre isotrope dans l'embedding space $(\mathbb{R}^d)$}


The choice of an embedding distribution used by a self-supervised learning method influences the performance on downstream learning tasks. Given a downstream task–such as linear regression or kernel density estimation–some embedding distributions require more training examples than others to attain an equivalent mean squared error loss. 

\iffalse
Self-supervised representations are often evaluated using %a small set of
%standardized downstream protocols, most notably 
linear probing, $k$-nearest neighbors
($k$-NN) regression or classification, and pixelwise dense prediction tasks such as semantic segmentation.
For a fixed number of training examples, the loss of each of these tasks is related to the geometric properties of the learned representation space.
%In particular, linear probing and $k$-NN constitute the two most elementary tests of
%representation quality, while segmentation performance largely depends on the same
%local and global geometric regularities.
\fi

The work of Balestriero and LeCun \yrcite{balestriero2025lejepaprovablescalableselfsupervised} makes the case for isotropic Gaussian embeddings by demonstrating their optimal performance in both linear probing (ordinary least-squares regression) and nonlinear probing ($k$-NN and Nadaraya-Watson kernel regression). Specifically, they show that isotropic embeddings (not necessarily Gaussian) minimize the Tikhonov-regularized loss of ridge regression models fit to an arbitrary target on the embeddings using the linear kernel. Moreover, they show that isotropic Gaussian embeddings minimize, for a fixed number of training examples, the integrated square bias term of the bias-variance decomposition of the mean-squared error loss of $k$-NN regression and Nadaraya-Watson kernel regression.  However, their proofs involve assumptions that rule out common choices of latent representations, such as spherical embeddings. For example, they linearize the integrated square bias term with a Euclidean Taylor expansion that imposes smoothness constraints on the embedding distribution and regression target function over $\mathbb{R}^d$ that fail for functions defined on the sphere (ibid., Lemmas 4 and 5). Moreover, their optimality results (ibid., Theorems 1 and 7-9) depend on the fact that the leading term of this expansion, the Euclidean Fisher information integral
$$\int_{\mathbb{R}^d} ||\nabla \log p(x)||_2^2 p(x) dx$$
is minimized by the Gaussian distribution (ibid., Lemma 6)–and, with additional scalar constraints on the distribution (ibid., Theorem 9), the isotropic Gaussian. But this integral is not defined when $p$ is, for instance, a uniform probability measure on the sphere $\mathbb{S}^{d-1}\subset \mathbb{R}^d$. The uniform measure on the sphere is singular with respect to the Lebesgue measure on the ambient Euclidean space $\mathbb{R}^d$ and does not have a probability density function with respect to the Lebesgue measure on $\mathbb{R}^d$.

But the integrated squared bias of $k$-NN regression and kernel density estimation models on general Riemannian manifolds has been studied in the literature using an expansion in covariant Taylor series, which does not impose these smoothness requirements in the ambient space \cite{henry2011knearestneighbordensityestimation, pelletier2005kernel}. When we ask the equivalent question about embeddings on general Riemannian manifolds rather $\mathbb{R}^d$–what embedding distribution minimizes the integrated squared bias of downstream learning tasks–we find that the leading term, which isotropic Gaussian distributions minimize over non-compact distributions in $\mathbb{R}^d$–disappears when we place a uniform distribution on a compact Riemannian manifold.



%Motivated by these recent theoretical analyses of optimal embedding distributions for linear
%probing \cite{balestriero2025lejepaprovablescalableselfsupervised}, 
%In this section, we seek optimal
%distributions of representations when embeddings are constrained to lie on a compact Riemannian manifold embedded in $\mathbb R^d$.  
Thus, we show that the uniform distribution on a compact Riemannian manifold in $\mathbb{R}^d$ optimally learns $k$-NN models from a given number of samples: it minimizes the integrated square bias. Moreover, any distribution that is isotropic in the ambient space is optimal (in the bias-minimizing sense) for linear probing. Putting these two results together identifies the sphere as the unique optimal compact, connected Riemannian manifold without boundary for these downstream learning tasks.

%and $k$-NN naturally leads to
%uniform (or isotropic) distributions on the underlying manifold, thereby providing a
%unified geometric principle for strong SSL representations.


\subsection{Linear Probing Optimality on Riemannian Manifolds}
Frozen self-supervised representations are often evaluated with linear probing. 
%Linear probing is a standard protocols for evaluating frozen
%self-supervised representations.
Given a fixed encoder $f_\theta:\mathcal X\to\mathbb R^d$ and a dataset
$\{x_n\}_{n=1}^{N}$, we denote by
$Z = [f_\theta(x_1),\dots,f_\theta(x_N)]^\top\in\mathbb R^{N\times d}$
the corresponding matrix of embeddings.
For arbitrary downstream targets $y\in\mathbb R^N$, linear probing consists in
 solving the ridge regression problem with the linear kernel
\cite{golub2000tikhonov}
\[
\hat\beta
=
\arg\min_{\beta\in\mathbb R^d}
\|y-Z\beta\|_2^2+\lambda\|\beta\|_2^2,
\]
where $\lambda\ge 0$ is the Tikhonov regularization parameter. %(This analysis generalizes immediately to the case with vector targets.)

The targets $y$ are unknown
during representation learning. The bias and variance of the estimator $\hat\beta$
depend only on the second-order statistics of the embeddings $Z$. 
%This observation enables a distributional analysis of representation optimality.
%In particular, the bias and variance of ridge regression with the linear kernel

Loosely speaking, for any target attribute $y$ and point $p$ in the latent space, the ability to find a direction $\beta$ such that the projections of the embeddings around $p$ onto $\beta$–i.e., $Z\beta$–follow the target $y$ suggests the embedding space is locally ``well-organized.'' A fixed direction $\beta$ may assume many meanings–i.e., follow different target attributes–throughout the embedding space. %An attribute may be specified by aggregating many indices $Z\beta_i$, weighting them by how well each direction follows the target attribute locally. 
But for targets $y$ for which the embedding representation is well-suited, there may be a single direction that exposes the attribute via a single-index model with identity link $y=Z\beta$. The bias and variance of a ridge regression estimate of such a global linear model given $N$ embeddings depends on the covariance matrix of the embeddings.

\begin{restatable}[Lemmas~1 and~2 of
\cite{balestriero2025lejepaprovablescalableselfsupervised}]{thm}{thm-linear}
\label{prop:lp_isotropy}
Assume that the embeddings $Z$ have finite second moments and fixed total energy
$\mathrm{tr}(\mathrm{Cov}(Z))$.
%Then, among all embedding distributions with the same energy, any distribution
%that minimizes
\cite{balestriero2025lejepaprovablescalableselfsupervised} show that isotropic embedding distribution (that is, distribution satisfying $\text{Cov}(Z)=\sigma^2 I$) minimizes the worst-case bias of the linear probe for Tikhonov regularization parameter $\lambda>0$ and the total variance of the linear probe for unbiased ($\lambda=0$) Tikhonov estimates of $\beta$.
%\begin{itemize}
%\item the worst-case bias of the linear probe for $\lambda>0$, and
%\item the total variance of the linear probe for $\lambda=0$,
%\end{itemize}
%is the isotropic one, i.e.\ the distribution whose covariance matrix is a scalar
%multiple of the identity. 
This result is unchanged when we constrain the distribution to lie on a compact Riemannian manifold.
\end{restatable}
\begin{proof} Given in Appendix, Section~\ref{appendix:proofs}.
\end{proof}

When encoder outputs are constrained to lie on a manifold
$\mathcal M\subset\mathbb R^d$, isotropy in the ambient latent space $\mathbb{R}^d$ requires a distribution $\mu$ supported on $\mathcal{M}$ such that $\mathrm{Cov}_{\mu}(Z) = \alpha I_d
\quad\text{for some }\alpha>0$. This condition does not uniquely
determine $\mu$: many non-uniform distributions on the same manifold may have isotropic covariance.

\iffalse
If the encoder outputs are constrained to lie on a manifold
$\mathcal M\subset\mathbb R^d$, embedding isotropy imposes a feasibility requirement on the
pair $(\mathcal M,\mu)$, namely that there exists at least one probability
measure $\mu$ supported on $\mathcal M$ such that
\[
\mathrm{Cov}_{\mu}(Z) = \alpha I_d
\quad\text{for some }\alpha>0.
\]
In other words, the representation manifold must support an \emph{isotropic}
embedding distribution in the ambient latent space $(\mathbb{R}^d)$. This condition does not uniquely
determine $\mu$: many non-uniform distributions on the same manifold may have isotropic covariance (for example, when $\mathcal{M}$ is the sphere $\mathbb{S}^{d-1}$, the uniform measure and the discrete measure on the standard $\mathbb{R}^d$ basis points both have isotropic covariance).  %provided the manifold assumes a compensatory form.
\fi

However, in Section~\ref{knn}, we show that uniform distributions minimize $k$-NN integrated squared-error bias. Combining these criteria–uniformity and isotropy in the ambient latent space–identifies the sphere as the optimal connected manifold without boundary that supports a uniform distribution.

\subsection{$k$-NN Optimality and Local Uniformity on Riemannian Manifolds}
\label{knn}

We now turn to the $k$-nearest neighbor ($k$-NN) evaluation protocol, another standard
benchmark in self-supervised learning.
In contrast to linear probing, which is extrinsic and global, $k$-NN probing is
intrinsically local and directly sensitive to the neighborhood structure induced by
the representation geometry.
As a result, $k$-NN performance is governed by the local regularity of the embedding
distribution on the underlying representation manifold.

For embeddings concentrating on a smooth Riemannian manifold $\mathcal M$,
recent results on $k$-NN density estimation on manifolds
\cite{henry2011knearestneighbordensityestimation} show that the bias of local $k$-NN
estimators is controlled by the Laplace--Beltrami operator $\Delta_{\mathcal M}$ applied
to the embedding density.
In particular, the leading term of the integrated squared bias (ISB) depends on the
functional
\begin{equation}
\int_{\mathcal M} \big(\Delta_{\mathcal M} p(x)\big)^2\, p(x)^{-4/m}\, d\mathrm{vol}(x), \label{eq:leading_functional}
\end{equation}
where $p$ denotes the density of representations on $\mathcal M$.

As established in Proposition~\ref{prop:uniform_minimizes_isb_henry}, this functional is
minimized only if $\Delta_{\mathcal M} p = 0$.
On a manifold without boundary, this condition implies that $p$ is
constant, so that the uniform distribution with respect to the Riemannian volume
uniquely minimizes the leading $k$-NN bias.

\begin{restatable}[Uniform density minimizes the leading term of the ISB]{thm}{isb}
\label{prop:uniform_minimizes_isb_henry}
Let $(\mathcal M,g)$ be a $d$-dimensional connected Riemannian manifold without boundary, with positive injectivity radius $\mathrm{inj}(\mathcal M)>0$ and with Riemannian volume measure $d\mathrm{vol}$. Suppose, moreover, that there exists $p_{\min},p_{\max}$ such that  $0<p_{\min}\le p(x)\le p_{\max}<\infty$ and that $\Delta_{\mathcal M}p \in L^2(\mathcal M,d\mathrm{vol})$.
Let $X_1,\dots,X_n$ be i.i.d.\ random variables on $\mathcal M$ with density $p$ w.r.t.\ $d\mathrm{vol}$.
Let $\hat p_n$ denote the $k_n$-NN \emph{kernel-type} density estimator defined in equation~(1) of
\cite{henry2011knearestneighbordensityestimation}. 
Assume the hypotheses of Theorem~3.2.2 in \cite{henry2011knearestneighbordensityestimation}, which govern the form of the kernel density estimator and target function.  
Define the integrated squared bias
\[
\mathrm{ISB}_n
:=
\int_{\mathcal M}\big(\mathbb E[\hat p_n(x)]-p(x)\big)^2\,d\mathrm{vol}(x).
\]
Then
\[
\mathrm{ISB}_n
=
\frac{C_0^2}{k_n}\!\int_{\mathcal M}\!\!\!\!\big(\Delta_{\mathcal M}p(x)\big)^2\,p(x)^{-4/d}\,d\mathrm{vol}(x)
\;+\;O\!\left(\frac{1}{k_n}\right)\!,
\]
for an explicit constant $C_0>0$ depending only on the kernel and on $d$.
Consequently, the leading term of $\mathrm{ISB}_n$ is minimized uniquely by the uniform density
$p\equiv \mathrm{vol}(\mathcal M)^{-1}$.
\end{restatable}

\begin{proof}
Given in Appendix~\cref{appendix:proofs}.
\end{proof}

$k$-NN regression is, in effect, kernel density estimation with a spatially varying bandwidth. The analysis of the fixed-bandwidth case was treated in \citep[Theorem 3.2]{pelletier2005kernel} and the proof that uniform distributions minimize the leading term of the integrated squared bias transfers immediately to this case. (That work assumes compactness, but only to bound the second-order term of the Taylor expansion of the target density on the manifold. In the case of a compact manifold, however, the uniform distribution eliminates this remainder.)


\subsection{Why LP + k-NN imply good segmentation}
Finally, we emphasize that dense prediction tasks such as semantic segmentation inherit
their difficulty from both global linear separability and local neighborhood structure.
Linear probes assess the global conditioning of representations, while $k$-NN evaluates
local smoothness and neighborhood consistency.
Segmentation combines both requirements at the pixel or patch level.

Therefore, a representation that is simultaneously optimal for linear probing and
$k$-NN must exhibit uniform, isotropic geometry at both global and local scales.
This precisely corresponds to representations whose distribution is uniform on the
underlying Riemannian manifold.
Such representations are thus expected to perform well across the full spectrum of
SSL evaluation protocols.

\subsection{Choice of a Canonical Representation Geometry}

The analyses above impose two complementary optimality requirements on the
representation distribution.
Linear probing optimality requires the existence of an embedding distribution
with isotropic ambient covariance in $\mathbb R^d$, while $k$-NN optimality
selects the uniform distribution on the underlying representation manifold.

To satisfy both criteria simultaneously, the representation manifold $\mathcal M$
must admit a probability measure that is
\begin{itemize}
\item uniform with respect to its intrinsic (Riemannian) volume, and
\item isotropic in the ambient space $\mathbb R^d$ of the latent embeddings on $\mathcal M$.
\end{itemize}
To satisfy the first requirement, $\mathcal{M}$ must be compact; to satisfy the second requirement, $\mathcal{M}$ must be invariant under the action of the orthogonal group. Stiefel manifolds are the prototypical $\mathrm{O}(d)$-homogeneous compact, connected manifolds without boundary and spheres $\mathrm{O}(d)/\mathrm{O}(d-1)$ are the simplest examples thereof. The Stiefel manifolds $\mathrm{O}(d)/\mathrm{O}(d-k)$ for $k\geq 2$ are more challenging to work with due to their non-trivial lower homotopy: these lower-dimensional ``holes'' mean they are not simply connected and that ensembles of points can have multiple Karcher means.

\iffalse
Among all possible choices, the simplest and most canonical solution is to take
$\mathcal M$ to be the hypersphere $\mathbb S^{d-1}\subset\mathbb R^d$ endowed with
the uniform (Haar) probability measure.

Indeed, the uniform distribution on $\mathbb S^{d-1}$ is intrinsically uniform and
induces an isotropic covariance matrix in the ambient space.
As such, it simultaneously satisfies the necessary conditions for linear probing
optimality and the sufficient and necessary conditions for $k$-NN bias optimality.

This choice provides a minimal and geometrically natural representation space that
is optimal with respect to the two most fundamental SSL evaluation protocols, and
therefore constitutes a principled target geometry for self-supervised
representations.
\fi




\section{Experiments}

\subsection{Experimental Setup}

\paragraph{Architectures.}
We follow the LeJEPA~\cite{balestriero2025lejepaprovablescalableselfsupervised} and
DINOv3~\cite{dinov3} evaluation protocols and consider Vision Transformers~\cite{ViT}
(ViT-S/B/L/G) and ConvNeXt~\cite{ConvNext} (S/B/L/G) backbones.
All architectures are taken directly from the DINOv3 implementation.
Unless otherwise specified, ViT-Large is used for ablation studies due to its
strong performance and stability.
For all backbones, we append a linear projection layer to map the encoder output
to a fixed embedding dimension of 512.
All comparisons with LeJEPA and DINOv3 are conducted using identical backbone
architectures and embedding dimensions.

\paragraph{Training Data and Views.}
All models are pretrained on ImageNet-1K~\cite{imagenet}.
Following LeJEPA~\cite{balestriero2025lejepaprovablescalableselfsupervised}, we adopt architecture-dependent view configurations.
For Vision Transformers, we use a multi-crop strategy with $V=8$ views, including two global views ($V_g=2$), as recommended in \cite{balestriero2025lejepaprovablescalableselfsupervised}, with global crops at resolution $224\times224$ and six local views at resolution $96\times96$.
For CNN backbones, we use two global views at resolution $224\times224$.
Data augmentation strategies follow the standard recipes introduced in SimSiam~\cite{simsiam} and further popularized by DINO~\cite{dinov1}, and are kept identical across all methods.
For DINOv3, we directly use the publicly released pretrained backbones provided
by the authors.

\paragraph{Projection Head.}
Unless stated otherwise, we use a $3$-layer MLP projection head with GELU activations, following standard practice in self-supervised learning \cite{dinov1}.
For ablation studies, we fix the hidden dimension to $2048$ and vary the output
dimension in $\{64,128,256,512\}$.
This design is motivated by the stability analysis reported in LeJEPA, which
shows that small projection heads act as effective regularizers without causing
collapse~\cite{balestriero2025lejepaprovablescalableselfsupervised}.
Hidden dimensions for large-scale comparisons follow standard backbone-dependent
settings.

\paragraph{Optimization.}
LeJEPA adopts AdamW~\cite{adamw} with linear warm-up and cosine learning-rate decay
as its standard optimization recipe.
However, LS-JEPA aims to simplify further self-supervised learning pipelines by
relying on principled optimization choices with clearer optimality properties.

Cosine annealing and weight-decay scheduling are widely used in SSL but remain
largely heuristic, with limited theoretical grounding.
To remove these empirically motivated components, we replace the standard AdamW
scheduler by \textit{AdamWFreeScheduler}~\cite{adamwfreescheduler}, which provides
a mathematically grounded alternative that eliminates the need for explicit
learning-rate decay.

Our default optimizer is AdamWFreeScheduler with linear warm-up only.
For ablation, we compare two variants:
(i) AdamWFreeScheduler with linear warm-up only, and
(ii) AdamW with linear warm-up followed by cosine annealing.
All other optimization hyperparameters are kept identical to isolate the effect of
the scheduler.

Following LeJEPA, we use a base learning rate of $10^{-4}$.
Weight decay is set to $5\times10^{-2}$ for ViT backbones and $5\times10^{-4}$ for
CNN backbones.
Bias and normalization parameters are excluded from weight decay.

\paragraph{Batch Size and Training Budget.}
Based on the stability analysis of LeJEPA~\cite{balestriero2025lejepaprovablescalableselfsupervised}, we fix the batch size to $B=512$ and
the number of slices to $|A|=1024$.
Unless otherwise specified, ablation experiments are conducted for 100 epochs.
Large-scale comparisons are performed for 400 epochs.

\paragraph{Evaluation Protocol.}
We evaluate learned representations using frozen-backbone linear probing and
$k$-NN classification on ImageNet-1K~\cite{imagenet}, following standard SSL practice.
Unless stated otherwise, evaluations are performed on backbone features before
the projection head.
All reported results are averaged over three random seeds.

---

\subsection{Ablation Study: Defining a Standard Training Recipe}

Our first set of experiments aims at defining a simple and robust default
training recipe.
We conduct an ablation study on ViT-Large pretrained for 100 epochs on
ImageNet-1K~\cite{imagenet}.

\paragraph{Optimizer Simplification.}
We compare AdamWFreeScheduler with linear warm-up against AdamW with
linear warm-up and cosine annealing.
This experiment isolates the impact of removing explicit learning-rate
scheduling, with the goal of simplifying the training pipeline.

\paragraph{Projection Head Dimension.}
Using the same setup, we evaluate projection head output dimensions in
$\{64,128,256,512\}$ while keeping the hidden dimension fixed to 2048.
This study allows us to quantify the regularization effect of small projection
heads and to select a default configuration.

Based on these ablations, we define a standard configuration that is used in all
subsequent experiments.

---

\subsection{Comparison with State-of-the-Art SSL Methods}

Using the standard configuration defined above, we compare our method against LeJEPA and DINOv3. 
We follow the architectural choices of DINOv3 and evaluate ViT-S/B/L with patch size 16 and ConvNeXt-S/B/L backbones.
All models are pretrained for $400$ epochs on ImageNet-1K~\cite{imagenet} using identical training budgets and data augmentations.

We report k-NN classification accuracy and frozen-backbone linear probing performance on ImageNet-1K~\cite{imagenet}.
This controlled comparison highlights the impact of our optimization simplification independently of architectural confounders.



\subsection{Evaluation Across Data Regimes}

To further analyze representation quality, we evaluate k-NN and linear probing
performance under varying amounts of labeled data.
We consider $1,2,5,10,100,1000$, and all samples per class on ImageNet-1K~\cite{imagenet}.
This analysis reveals how quickly each method adapts in low-data and moderate-
data regimes.

---

\subsection{Representation Analysis and Visualization}

We analyze the structure of the learned representations using dimensionality
reduction techniques.
We present PCA visualizations of last-layer features obtained with our method,
and compare 2D t-SNE embeddings across LeJEPA, DINOv3, and our approach.
These visualizations qualitatively illustrate differences in cluster compactness
and semantic separation.



\subsection{Downstream Semantic Segmentation}

Finally, we evaluate the transferability of learned representations to dense
prediction tasks.
We compare LeJEPA, DINOv3, and our method on semantic segmentation using the
ADE20K dataset.
All models use frozen pretrained backbones and identical segmentation heads,
allowing for a fair comparison of representation quality.



\section{Optimality Criteria for Self-Supervised Representations}
\label{OptimalityRepresentation}

A central goal of SSL is to learn representations that support a wide range of downstream tasks with minimal supervision.
In practice, representation quality is most commonly assessed using a small set of standardized evaluation protocols, among which \emph{linear probing} and \emph{$k$-nearest neighbors ($k$-NN)} play a central role~\cite{simclr,byol,dinov1}.

Beyond their empirical popularity, these two protocols capture complementary and fundamental aspects of representation geometry.
In this section, we show that requiring strong performance on both linear probing and $k$-NN imposes strong and interpretable constraints on the distribution of learned representations.
In particular, these criteria uniquely identify the uniform distribution on the hypersphere as the optimal representation geometry under mild assumptions.

\subsection{Why Linear Probing and $k$-NN Matter}

Linear probing evaluates representations by fitting a linear predictor on top of frozen embeddings~\cite{simclr}.
Given embeddings $z_i \in \mathbb{R}^d$ and targets $y_i$, linear probing amounts to solving a ridge regression problem~\cite{golub2000tikhonov}
\[
\hat{\beta}
=
\arg\min_{\beta \in \mathbb{R}^d}
\sum_{i=1}^N (y_i - \langle z_i, \beta \rangle)^2 + \lambda \|\beta\|_2^2,
\]
which is equivalent, under standard assumptions, to linear classification with cross-entropy loss when the number of classes is fixed and the embeddings are well conditioned~\cite{zhang2004statistical}.
Thus, linear probing measures the ability of the representation to support \emph{globally linear} readouts.

In contrast, $k$-NN evaluation is a purely nonparametric and local method~\cite{hastie2009elements}.
Predictions are made by aggregating the labels of nearby points in the representation space, making $k$-NN directly sensitive to the local geometry and density of the embedding distribution.
Good $k$-NN performance therefore requires that semantic neighborhoods are well-structured and uniformly sampled.

Together, linear probing and $k$-NN probe complementary properties of representations: linear probing tests global conditioning and alignment, while $k$-NN tests local regularity and neighborhood consistency.
A representation that performs well on both must therefore exhibit strong global and local geometric structure.

\subsection{Optimality of Self-Supervised Representations}

We now summarize the optimality requirements imposed by standard downstream evaluation
protocols.
Throughout this section, we adopt a worst-case, distributional notion of optimality:
since downstream targets are unknown at representation learning time, a representation
is considered optimal if it minimizes the bias of downstream estimators uniformly over
all possible targets.

Two evaluation protocols play a central role in self-supervised learning: linear
probing and $k$-nearest neighbors ($k$-NN).
Although simple, they capture complementary and fundamental aspects of representation
geometry.

Linear probing evaluates the ability of a representation to support global linear
readouts.
As shown in Appendix~\ref{appendix:proofs}, minimizing the bias of linear probing
requires the representation to be \emph{isotropic} in the ambient space ($\mathbb{R}^d$), meaning that no direction is privileged.

In contrast, $k$-NN evaluation is intrinsically local.
As shown in Appendix~\ref{appendix:proofs}, minimizing the bias of $k$-NN
estimators requires the representation to be \emph{uniformly distributed} on its
support.
This, in turn, forces the support of the representation to be a compact Riemannian
manifold without boundary.

Taken together, these two requirements severely restrict the possible geometry of
optimal representations.
Uniformity is required intrinsically on the representation manifold, while isotropy is
required extrinsically in the representation ambient space ($\mathbb{R}^d$).

Under a mild connectivity assumption—namely that the representation manifold forms a
single connected component—these constraints admit a unique solution.

\begin{theorem}[Canonical optimal representation geometry]
\label{thm:canonical_geometry}
Assume that self-supervised representations are supported on a connected Riemannian
manifold without boundary, embedded in $\mathbb{R}^d$.
If a representation is simultaneously optimal for linear probing and $k$-nearest neighbors evaluation, then it must be uniformly distributed on the hypersphere $\mathbb{S}^{d-1}$.
\end{theorem}

The proof, given in Appendix~\ref{appendix:proofs}, follows from three steps:
(i) linear probing optimality enforces ambient isotropy,
(ii) $k$-NN optimality enforces uniformity on a compact manifold, and
(iii) under connectivity and the absence of boundary, these two conditions uniquely
characterize the hypersphere.

